DiffMix: Diffusion Model-based Data Synthesis for Nuclei Segmentation and Classification in Imbalanced Pathology Image Datasets

Nuclei segmentation and classification is a significant process in pathology image analysis. Deep learning-based approaches have greatly contributed to the higher accuracy of this task. However, those approaches suffer from the imbalanced nuclei data composition, which shows lower classification performance on the rare nuclei class. In this paper, we propose a realistic data synthesis method using a diffusion model. We generate two types of virtual patches to enlarge the training data distribution, which is for balancing the nuclei class variance and for enlarging the chance to look at various nuclei. After that, we use a semantic-label-conditioned diffusion model to generate realistic and high-quality image samples. We demonstrate the efficacy of our method by experiment results on two imbalanced nuclei datasets, improving the state-of-the-art networks. The experimental results suggest that the proposed method improves the classification performance of the rare type nuclei classification, while showing superior segmentation and classification performance in imbalanced pathology nuclei datasets.

==> f8_rebuttal.tex <==
\begin{enumerate}

\begin{center}
    \Large\bfseries [MICCAI'23] Rebuttal Letter
\end{center}

\vspace{0.5\baselineskip}

\begin{center}
    https://docs.google.com/document/d/1PsH8F3nDDbRZ0g9uYPxKhJHdr-Txb6gElZ-GwkVqoW4/edit
\end{center}

\vspace{1\baselineskip} % Adjust the vertical spacing

% \title{[MICCAI'23] Rebuttal Letter}
% \maketitle

% \begin{titlepage}
%     \centering
%     \vspace*{\baselineskip} % Adjust the vertical spacing
    
%     \Large\bfseries [MICCAI'23] Rebuttal Letter
    
%     \vspace{0.5\baselineskip} % Adjust the vertical spacing
    
%     % \Large Subtitle or additional information
    
%     % \vspace{2\baselineskip} % Adjust the vertical spacing
    
%     % \Large Author Name
    
%     % \today % Optionally, add the current date
    
%     % \vspace*{\baselineskip} % Adjust the vertical spacing
% \end{titlepage}

% \centering{[MICCAI'23] Rebuttal Letter}

\item{
\textbf{[R2, R4] Need comparison with more related works, such as CutMix, CutOut and GAN-based methods} \\

We mainly compared our method to one of the most recent SOTA methods, GradMix [MICCAI22].

[CutMix and CutOut] They are rather outdated methods and did not perform better compared to the baseline (HoVer-Net). CutMix showed lower scores (-2.5\% to -0.5\% per metric), 
while CutOut performed similarly in GLySAC and slightly better in CoNSeP (-0.3\% to +1\% per metric). Due to space limitations, we excluded CutMix and CutOut from the text.

[GAN-based methods] SDM generates more realistic images compared to SOTA GAN methods. We also confirmed that the Pix2Pix method performed worse in CoNSeP (-3\% to -0.6\% per 
metric and much lower $F_M$). Therefore, we did not directly compare to GAN approaches.
} \\

\item{
\textbf{[R1, R2, R3] Need detailed description of data sampling and mask design} \\

“Enlarging maps” perturb the positions of nuclei instances to diversify datasets. As for the comparison with the smart sampling strategy, our method can handle imbalance 
at the instance level more precisely in the balancing map by removing or adding individual nuclei while the sampling strategy can be done at the image level by selecting 
more or fewer images to reduce class imbalance in the training data. We will clarify the text on the methodology description.
} \\

\item{
\textbf{[R1, R2] Limited Novelty} \\

We introduce a unique combination of semantic diffusion models and virtual masks to synthesize realistic data, offering a novel solution for addressing data imbalance 
in pathology nuclei analysis. Moreover, our approach performs superior across SOTA networks and significantly improves the classification score for the rarest nuclei type 
($F_M$) in CoNSeP (Table 1). To the best of our knowledge, this is the first attempt to employ the diffusion model to address the semantic data imbalance in pathology.
} \\

\item{
\textbf{[R2] Discrepancies in GradMix performance from the original paper} \\

Replicating the exact results in the GradMix paper was impossible due to randomness in the GradMix algorithm, hyperparameters of SONNET, and random splits of the train set. 
We believe a direct comparison between our result and the numbers from the GradMix paper is not accurate to assess the performance difference. 
Instead, we conducted all the experiments under the same environment; We used the official codes (HoVer-Net, SONNET, and GradMix), conducted cross-validation, 
maintained consistent hyperparameters for the baseline networks, and carefully splitted data to include all nuclei types in each fold. 
The only difference between the methods was the type of synthesized data (by GradMix or DiffMix) in the training set. 
The results demonstrated that DiffMix consistently outperforms GradMix across SOTA baselines, particularly on the CoNSeP dataset (Table 1).
} \\

\item{
\textbf{[R1] Model dependency on training data distribution} \\

Diffusion models, unlike GANs that directly generate images from noise, progressively refine a noise vector to an image. 
Generating a new image from a noise-added input image as in our method, model dependency on the training data distribution can be mitigated to a certain degree.
} \\

\item{
\textbf{[R4] Limited performance gain on segmentation} \\

Due to the baseline networks having separate branches for segmentation and classification, our semantic balancing strategy had a minor effect on segmentation 
(because no semantic difference in foreground labels) but significantly improved classification.
} \\

\item{
\textbf{[R2, R3] Source code} \\

We will release the source code upon acceptance.
} \\

\item{
\textbf{[R1] Reference of pretrained SDM} \\

We pretrained SDM by ourselves (sec. 3.2), but will clarify in the text.
} \\

\item{
\textbf{[R2] Training time} \\

Training SDM took around 13 hours. A 256x256 image synthesis took approximately 20 seconds.
} \\

\item{
\textbf{[R2] Trade-off between computational overhead and practical benefits} \\

The major overhead is in the training, so we believe the usability at inference may not be degraded much while the high quality image from diffusion models is practically beneficial.
} 



\end{enumerate}
